A Simple and Efficient Lagrange Multiplier Based Mixed Finite Element for Gradient Damage

A novel finite element formulation for gradient-regularized damage models is presented which allows for the robust, efficient, and mesh-independent simulation of damage phenomena in engineering and biological materials. The paper presents a Lagrange multiplier based mixed finite element formulation for finite strains. Thereby, no numerical stabilization or penalty parameters are required. On the other hand, no additional degrees of freedom appear for the Lagrange multiplier which is achieved through a suitable FE-interpolation scheme allowing for static condensation. In contrast to competitive approaches from the literature with similar efficiency, the proposed formulation does not require cross-element information and thus, a straightforward implementation using standard element routine interfaces is enabled. Numerical tests show mesh-independent solutions, robustness of the solution procedure for states of severe damage and under cyclic loading conditions. It is demonstrated that the computing time of the gradient damage calculations exceeds the one of purely elastic computations only by an insignificant amount. Furthermore, an improved convergence behavior compared to alternative approaches is shown.

==> sec_00_title.tex <==

%========================================================================
%          ***  First Page of Paper  ***
%========================================================================
\thispagestyle{empty}

% heading -------------------------------
% \begin{figure}[htb]
% \unitlength1cm
% \begin{picture}(21,0.5)
% % \put(-1.9, 0.15){\includegraphics[width=57mm]{\logopath/TU_logo_sw.eps}} % for black&white docs
% \put(-1.9, 0.15){\includegraphics[width=57mm]{\logopath/TU_logo_hks41.eps}} % for docs in color
% \put( 0.0,-0.35){\textcolor{\headercolor}{\vrule width15.5cm height.5pt}}
% \put( 0.0,-0.73){\scriptsize{\textcolor{\headercolor}{\sffamily\textbf{Fakult\"at Bauingenieurwesen} Institut f\"ur Mechanik und
% Fl\"achentragwerke}}}
% \put( 0.0,-0.85){\textcolor{\headercolor}{\vrule width15.5cm height.5pt}}
% \end{picture}
% \end{figure}

\begin{figure}[htb]
\unitlength1cm
\begin{picture}(21,1.25)
% \put( 13.0, 0.0){\includegraphics[width=37.5mm]{\logopath/RUB_label_2000x2000.eps}}
% \put(-1.75, 2.25){\includegraphics[height=3.125mm]{\logopath/RUB_schriftzug.eps}}
% \put(-1.75, 2.15){\includegraphics[width=65mm]{\logopath/RUB_schriftzug.eps}}
% \put(-1.80, 1.6){\textcolor{\headercolor}{\sffamily\textbf{Chair of Continuum Mechanics}}}
% \put(-1.77, 1.1){\textcolor{\headercolor}{\sffamily{Prof.~Dr.-Ing.~habil. Daniel Balzani}}}

\put(-2.0, 2.45){\textcolor{\headercolor}{\sffamily\textbf{Chair of Continuum Mechanics}}}
\put(-2.0, 1.90){\textcolor{\headercolor}{\sffamily{Prof.~Dr.-Ing.~habil. Daniel Balzani}}}
\put(12.0, 1.6){\includegraphics{\logopath/RUB_logo_blau_4c.eps}}
\end{picture}
\end{figure}

% ------------------------------------------

\vspace{3cm}

{\Huge
This is the Title of the Manuscript\\
} 

\vspace{5mm}

Author 1, Author 2, Author 3,...

\vfill

==> tex/sec_02_temp.tex <==
\section{Continuum mechanical framework\label{s:framework}}
This section covers the continuum mechanical framework, in which the proposed formulation of the following section is embedded.
First, section \ref{ss:kinematics} introduces some notation and finite strain kinematics used throughout this contribution.
In section \ref{ss:thermo} the thermodynamic framework is given and in section \ref{ss:cont_damage_mech} finite strain gradient damage fundamentals are presented. 

\subsection{Kinematics\label{ss:kinematics}}
$\phi:\B\rightarrow \Bt$

$\bF\defeq\p{\bX}\phi=\bu+\bone$

$\sed(\bF,\iv)\defeq (1-D(\iv))\sed_0(\bF)$

$D:\bR^+\rightarrow [0,1)$ and the continuous monotonic decreasing function $\giv:\R^+\rightarrow (0,1] $ models the material softening due to damage evolution with $g(0)=1$ being the completely intact and $g\rightarrow 0$ approaching the completely damaged material state.

\subsection{Thermodynamics\label{ss:thermo}}
The most fundamental framework in which the follwing formulations are embedded are the first and second law of thermodynamics
\eb
 \int_{t_n}^{t} \dot{\Pi} \delta t = 0 \qquad
 \text{and} \qquad
 \int_{t_n}^{t} \dot{\Gamma} \delta t \geq 0, 
 \footnote{$\dot{(\bullet)}\defeq\p{t}{(\bullet)}$ denotes the time derivative.}
 \label{e:thermo_laws_fundamental}
\ee
which need to be fulfilled for any process time interval $[t_n,t]$.
Here $\Pi$ denotes the total energy of $\B$ and $\Gamma$ the total entropy of $\B$.
In the context of this contribution process conditions are assumed do be adiabatic, isothermal and quasi static.
% In the context of this contribution process conditions are assumed do be adiabatic (no heat transfer), isothermal (no temperature change) and quasi static (no change of kinetic energy).
Thus, the energy potential simplifies to the sum of internal energy $\Pi_{\mrm{int}}$ and external work $\Pi_{\mrm{ext}}$.

\subsection{Gradient Damage Fundamentals\label{ss:cont_damage_mech}}


The functionals read:
% potentials
\begin{align}
% \Pi &= \int_{\B} (1-\dv(\iv)) \sed_0 + \frac{\nlpar}{2} \Grad\iv \scp \Grad\iv + \mathcal{D}_{\mrm{diss}}(\iv) \dX
\Pi &= \underbrace{\int_{\B} \sed(\bF,\iv) +\diss(\iv,\Grad\iv) \dX}_{\Pi_{\mrm{int}}}
\underbrace{-\int_{\B}  \bu \scp \bbf \dX - \int_{\dBN} \bu \scp \bt \dA }_{\Pi_{\mrm{ext}}}
\label{e:total_energy_potential}\\
\Gamma &= \int_{\B} \diss(\iv,\Grad\iv) \dX,
\label{e:total_dissipation_potential}
\end{align}
where the integrand of the internal energy consists of the sum of the free elastic energy $\sed(\bF,\iv)$ and the internal dissipation $\diss(\iv,\Grad\iv)$ due to evolution of the microstructure both as functions of the damage variable $\iv$.
% \footnote{Note that $\iv$ is also referred to as phase field variable (cite de lorenzis and other phase field lit.)}
% The free elastic energy $\sed$ and the dissipation function $\diss$ are given by
% \begin{align}
% \sed(\bF,\iv) &\defeq \giv\, \sed_0(\bF),
% \label{e:free_int_energy} \\
% \diss(\iv,\Grad\iv) &\defeq \wiv + \frac{\nlpar}{2} \Grad\iv \scp \Grad\iv
% \label{e:diss}
% \end{align}
% respectively.
% Here, $\sed_0$ is the virtually undamaged hyperelastic energy function %, $\iv$ denotes the damage variable%
% \footnote{Note that $\iv$ is also referred to as phase field variable (cite de lorenzis and other phase field lit.)}
% and the continuous monotonic decreasing function $\giv:\R^+\rightarrow (0,1] $ models the material softening due to damage evolution with $g(0)=1$ being the completely intact and $g\rightarrow 0$ approaching the completely damaged material state.
Further, $\diss$ is a continuous monotonic increasing function $\iv$ and $\Grad\iv$ (with $\p{\iv}{\diss}\geq 0 and $
% \footnote{$(\bullet(\square))'\defeq \p{\square}{(\bullet)}$ denotes the scalar first derivative operator.}
% and $\displaystyle\lim_{\iv\rightarrow \infty}\wiv=\infty$ (cf. \cite{GerDeL:2019:opi})) so that the second law \eqref{e:thermo_laws_fundamental}$_2$ is always fulfilled if $\dot{\iv}\geq0$, since with the nonlocal constant $\nlpar>0$ the gradient term in \eqref{e:diss} is always greater than zero.
For further reading cf. \cite{GerDeL:2019:opi,MieAldRai:2016:pfm,MieWelHof:2010:tcp}.
%
% The latter is a continuous monotonic increasing function $\wiv:\R^+\rightarrow\R^+$ (with $\wiv'\geq 0$
% \footnote{$(\bullet(\square))'\defeq \p{\square}{(\bullet)}$ denotes the scalar first derivative operator.}
% and $\displaystyle\lim_{\iv\rightarrow \infty}\wiv=\infty$) so that the second law \eqref{e:thermo_laws_fundamental}$_2$ is always fulfilled if $\dot{\iv}\geq0$.
% Meanwhile, the gradient enhanced free elastic energy $\sed$ is given by
% % \eb
% % \sed(\bF,\iv,\Grad\iv) \defeq \giv\, \sed_0(\bF)  + \frac{\nlpar}{2} \Grad\iv \scp \Grad\iv,
% % \label{e:free_int_energy}
% % \ee
% where $\sed_0$ is the virtually undamaged hyperelastic energy function %, $\iv$ denotes the damage variable%
% % \footnote{Note that $\iv$ is also referred to as phase field variable (cite de lorenzis and other phase field lit.)}
% and the continuous monotonic decreasing function $\giv:\R^+\rightarrow (0,1] $ models the material softening due to damage evolution with $g(0)=1$ being the completely intact and $g\rightarrow 0$ approaching the completely damaged material state.
% Here, $\nlpar$ is a nonlocal material parameter.
% % The volume specific internal energy $\varepsilon\defeq \sed+\diss$ is the sum of the free elastic energy $\sed$ and internal dissipation $\diss$ due to evolution of the microstructure.
% % In the present case the latter is modeled in terms of the continuous monotonic increasing function $\wiv:\R^+\rightarrow\R^+$ (with $\wiv'\geq 0$
% % \footnote{$(\bullet(\square))'\defeq \p{\square}{(\bullet)}$ denotes the scalar first derivative operator.}
% % and $\displaystyle\lim_{\iv\rightarrow \infty}\wiv=\infty$).
% %
% %
Insertion of \eqref{e:total_energy_potential}-\eqref{e:total_dissipation_potential} into \eqref{e:thermo_laws_fundamental} yields the following strong form of the gradient damage problem:
Find $\iv$ and $\bu$ such that

\begin{align}
 -\Div\bP&=\bbf \text{ in } \B \label{e:bal_lin_mom_orig}\\
 \bP \nv &= \bt \text{ on } \dBN \label{e:cauchy_theorem_orig}\\
%  \big( \giv' \sed_0 -\nlpar \Delta\iv + \wiv' \big)\,\dot{\iv} &= 0 \text{ in } \B 
 \big( \p{\iv}{\sed}-\Div\p{\Grad\iv}{\diss} + \p{\iv}{\diss} \big)\,\dot{\iv} &= 0 \text{ in } \B 
 \label{e:strong_form_phasefield_eq_origin}\\
%  \Grad\iv \nv &= 0 \text{ on } \dB \\
 (\p{\Grad\iv}{\diss})\smpc \nv &= 0 \text{ on } \dB \\
 \dot\iv &\geq 0 \text{ in } \B
 \label{e:ineq_constraint_origin}
\end{align}
Here, $\Delta(\bullet)$ denotes the Laplace operator, $\bP\defeq\p{\bF}{\sed}= \giv\,\p{\bF}{\sed_0}$ denotes the first Piola-Kirchhoff stress tensor. %and $\delta(\bullet)=\bullet\vert_{t_1}-\bullet\vert_{t_0}$ denotes the change of field value over arbitrary process time period aka test function.
Equations \eqref{e:strong_form_phasefield_eq_origin} and \eqref{e:ineq_constraint_origin} can be written as Karush-Kuhn-Tucker conditions \cite{KuhTuc:1951:np} (see also \cite{Ber:1982:coa}) for the solution of optimization problems with inequality constraints:
\eb
 \yieldf \leq 0  ,\quad  \dot\alpha \geq 0 \quad \text{and}\quad  \yieldf\, \dot\iv = 0 \qquad \text{with} \quad
 \yieldf\defeq\yieldf(\bF,\iv,\Grad\iv)= -\p{\iv}{\sed}+\Div\p{\Grad\iv}{\diss} - \p{\iv}{\diss}.
%  \yieldf \defeq  \underbrace{-\giv' \sed_0}_{-\p{\iv}{\sed}} +\nlpar \Delta\iv - \wiv',
 \label{e:kkt_origin}
\ee
where the corresponding Lagrangian in the present case is the elastic potential $\Pi$ itself.
Thus, problem \eqref{e:bal_lin_mom_orig}-\eqref{e:ineq_constraint_origin} is identical to finding $\bu,\iv$ such that
\eb
\qquad \Pi \Rightarrow \min_{\bu,\iv}, \qquad \text{subject to} \qquad \dot{\iv}\geq 0\ (\text{at each point in }\B)%\yieldf \leq 0\ (\text{at each point in }\B).
\label{e:opt_probl_origin}
\ee
% The inequality condition is then incorporated in the following sense:
% \begin{align}
%  \text{If } \yieldf > 0 , \text{ find } \iv \text{ such that } \yieldf=0
% \end{align}

% In local damage formulations ...cf... a numerical approach to the solution of the problem corresponding to \eqref{e:opt_probl_origin} is to discretize the weak form of the balance of linear momentum  with finite elements

% \begin{remark}
% \coljr{EDIT THIS SECTION}
%  Note, that \eqref{e:kkt_origin} is equivalent to the following. 
%  Let $\beta$ denote the thermodynamic force and $Y$ denote the energy release rate given by
%  \begin{align}
%  \beta &= -\p{\iv}{\sed}\defeq -\giv'\sed_0+\nlpar \Delta\iv & \text{(driving force)} \quad\text{and} \\
%  Y &\defeq \wiv'                             & \text{(energy release rate)}.
%  \end{align}
%  Then, in the representation of classical discontinuous damage formulations ...cite... the release of energy over the process time intervall $[t_0,t_1]$ in terms of the damage variable $\iv$ is given by
%  \eb
%  Y(\iv) = \sup_{t_0<t<t_1}\{\beta(\iv),0\} \quad \text{and its derivative} \quad
%  \dot{Y} = \begin{cases}
%               \dot{\beta} & \text{if } \yieldf \leq 0 \\
%               0             & \text{else}.
%              \end{cases}
%  \label{e:update_condition_origin}
%  \ee
% %  where $[t_0,t_1]$ is some time intervall
% 
% % \begin{align}
% %  \text{Damage evolution:} &\text{If } \yiedf > 0,
% %  \text{No evolution:}     &\text{If } \beta\leq Y
% % \end{align}
% 
% 
% 
% \end{remark}

By introducing $\drivingforce\defeq-\p{\iv}{\sed}$ as the driving force and $r(\iv,\Delta\iv)\defeq \wiv' - \nlpar \Delta\iv $ as energy release (cf ...), the damage evolution corresponds to the following relations:
\eb
\dot{r} =
\begin{cases}
\dot{\beta} \quad\text{if } \yieldf \geq  0 & \text{(damage evolution)}\\
0  \quad\text{else } & \text{ (no evolution)}
\end{cases}
\qquad\Leftrightarrow\qquad
\dot{\iv} =
\begin{cases}
\underset{t}{\operatorname{argmin}}\{\yieldf\} \\
0
\end{cases}
\label{e:evolution}
\ee
\coljr{Further edit...}
The common numerical approach in local continuum damage formulations ($\nlpar=0$, no gradient enhancement term) ...cf.cite... is to discretize $\bF(\Grad\bu^h)$ with finite elements, while the evolution condition \eqref{e:evolution} is resolved locally at the integration point level.
% evaluation of the update condition \eqref{e:kkt_origin} (or \eqref{e:update_condition_origin}) is performed at the material point level.
Therefore, the variable $\iv^h$ is stored as history parameter.
However, with gradient enhancement this is not straitforwardly possible due to the appearance of the Laplace operator in $\yieldf$.
A remedy is to either use a discretization of $\iv$, which possesses interelement continuity so that an approximation of the gradient enhancement is possible ...cite junker etc/ lorenzis...
or to use a mixed formulation ...cite mixed formulations....



